Towards a Diagrammatic Analogue of the Reshetikhin-Turaev Link Invariants

By considering spaces of directed Jacobi diagrams, we construct a diagrammatic version of the Etingof-Kazhdan quantization of complex semisimple Lie algebras. This diagrammatic quantization is used to provide a construction of a directed version of the Kontsevich integral, denoted $Z_EK$, in a way which is analogous to the construction of the Reshetikhin-Turaev invariants from the R-matrices of the Drinfel'd-Jimbo quantum groups. Based on this analogy, we conjecture (and prove in a restricted sense) a formula for the value of the invariant $Z_EK$ on the unknot. This formula is simpler than the Wheels formula of [BGRT], but the precise relationship between the two is yet unknown.

==> draws/BC.tex <==
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
{\renewcommand{\dashlinestretch}{30}
\begin{picture}(1116,951)(0,-10)
\path(483,843)(483,93)
\thicklines
\path(33,93)(1083,93)
\blacken\path(903.000,33.000)(1083.000,93.000)(903.000,153.000)(903.000,33.000)
\path(33,843)(1083,843)
\blacken\path(903.000,783.000)(1083.000,843.000)(903.000,903.000)(903.000,783.000)
\end{picture}
}


==> draws/OvrX.tex <==
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
{\renewcommand{\dashlinestretch}{30}
\begin{picture}(924,1239)(0,-10)
\path(12,12)(912,1212)
\blacken\path(864.000,1098.000)(912.000,1212.000)(816.000,1134.000)(818.400,1087.200)(864.000,1098.000)
\path(912,12)(492,572)
\path(432,652)(12,1212)
\blacken\path(108.000,1134.000)(12.000,1212.000)(60.000,1098.000)(105.600,1087.200)(108.000,1134.000)
\end{picture}
}


==> draws/UndrX.tex <==
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
{\renewcommand{\dashlinestretch}{30}
\begin{picture}(924,1239)(0,-10)
\path(912,12)(12,1212)
\blacken\path(108.000,1134.000)(12.000,1212.000)(60.000,1098.000)(105.600,1087.200)(108.000,1134.000)
\path(12,12)(432,572)
\path(492,652)(912,1212)
\blacken\path(864.000,1098.000)(912.000,1212.000)(816.000,1134.000)(818.400,1087.200)(864.000,1098.000)
\end{picture}
}

